2D-2FA: A New Dimension in Two-Factor Authentication

We propose a two-factor authentication (2FA) mechanism called 2D-2FA to address security and usability issues in existing methods. 2D-2FA has three distinguishing features: First, after a user enters a username and password on a login terminal, a unique $\textit{identifier}$ is displayed to her. She $\textit{inputs}$ the same identifier on her registered 2FA device, which ensures appropriate engagement in the authentication process. Second, a one-time PIN is computed on the device and $\textit{automatically}$ transferred to the server. Thus, the PIN can have very high entropy, making guessing attacks infeasible. Third, the identifier is also incorporated into the PIN computation, which renders $\textit{concurrent attacks}$ ineffective. Third-party services such as push-notification providers and 2FA service providers, do not need to be trusted for the security of the system. The choice of identifiers depends on the device form factor and the context. Users could choose to draw patterns, capture QR codes, etc. We provide a proof of concept implementation, and evaluate performance, accuracy, and usability of the system. We show that the system offers a lower error rate (about half) and better efficiency (2-3 times faster) compared to the commonly used PIN-2FA. Our study indicates a high level of usability with a SUS of 75, and a high perception of efficiency, security, accuracy, and adoptability.

==> discuss.tex <==
%!tex root = main.tex

\section{Discussion} %and Future Work}
\label{sec:discussion}

%\subsection{Orthogonal Defensing Mechanisms}  

\nsha{Discuss DoS attacks in this section.}

\mypara{Phishing Attacks}  2FA is mainly used to strengthen security against online password guessing attacks. 
The aim is to prevent an attacker who knows or guesses the password from authenticating
unless access to the secondary device is proved. Some 2FA approaches, such as FIDO
\cite{fidou2f}, claim to prevent man-in-the-middle phishing attacks against 2FA  by binding the 
keys to the origin. \nsha{binding the keys or signatures?} Replaying the challenge to the client would not help the 
man-in-the-middle phishing attacker to login successfully because the device 
also signs the origin and the channel ID, which can be verified by the server. 
While this approach prevents the PIN man-in-the-middle phishing attack, 
it does not prevent the attacker from learning the password (which could have 
been reused on other services with no 2FA in place). \nsha{why man-in-the-middle?} \nsha{why bring passwords here?} Besides, it requires modification on the client 
browser. 
We do not intend to prevent phishing attacks and assume that such attacks should \shashank{should or could?} be prevented 
on the password level (for example, by using password managers that generate origin-specific password \cite{pwdhash}).

\shashank{This makes me wonder about a different thing. What if in FIDO, I have different signing keys for different domains? Is this the case by default? Then, is there any need to sign the origin, etc.?}

\mypara{Offline Dictionary Attacks} Some other 2FA schemes, such as \cite{ndss-2014, pkc-2018} attempt to solve the offline dictionary 
attack issues in which an attacker compromises 
the server and runs an offline attack to retrieve the securely stored password. 
While we do not directly propose any method to secure the password authentication against 
offline dictionary attacks, integration with schemes, such as the one proposed in \cite{ndss-2014}, is trivial, 
to resist these attacks. 

% \mypara{Pattern Guessing} We do not require the pattern to be selected from a large dictionary since 
% guessing the pattern does not impose any security threat in our approach. In fact, the PIN and the pattern can 
% be communicated in clear.  An attacker who knows the password needs to guess both the PIN 
% and the pattern to successfully login to the system.
% Since in computation of the PIN, both pattern and secret key are involved, even after guessing the pattern,  
% computing the PIN requires knowledge of the secret key, and guessing the PIN is not feasible since the
% PIN can be long thanks to the automated transfer. 

% \shashank{We don't need to have a separate paragraph on this. This is a part of the security analysis. But it may be of value to talk about this separately (or multiple times).}


\mypara{Fallback Mechanism} Our approach assumes that the device can connect to the server (e.g., over the internet).  But in case the device loses connectivity, we can fall back to an \stfa\ like method. After the user inputs the \id on the device, the computed PIN will be displayed to her. She can manually copy the PIN to the client terminal, which would then be transferred to the server. 

% a direct communication between the device and the server. In case the device loses connectivity, we can still fall back to \stfa\ in which the user draws the pattern on the
% device and the device displays the PIN. The user can manually copy the PIN on the client to be transferred to the server
% similar to the traditional \stfa. 
% \shashank{But the length of the PIN may be a problem.} 

%\textbf{Denial of Service:} 

%\subsection{Limitation of this work} 
% \mypara{QR codes} One may wonder if drawing patterns in \ptfa can be replaced by scanning QR codes. (QR codes are used by WhatsApp Web \cite{whatsapp-desktop}, Tozny \cite{galois-qr-code}, etc.\ for authentication.) While this may seem appealing at first from a usability perspective, a closer look would reveal several problems. First of all, while a touch-screen (for drawing a pattern) is available on a myriad of devices these days, camera (for scanning) is not so universal. For e.g., smartwatches, smart-home devices, car-dashboard screens, etc.\ generally have touch-screens, but most of them do not have any camera. Adding camera to IoT devices also raises privacy concerns, so manufacturers tend to be very careful. Secondly, camera needs to be pointed at QR code, which could be difficult or even impossible (e.g., a car-dashboard screen). Finally, a QR code could embed a lot of information, which could be used to exploit weaknesses in scanning/2FA apps.



==> usability.tex <==
\section{Discussion and Future Work}



